Process Model Forecasting Using Time Series Analysis of Event Sequence Data

Process analytics is an umbrella of data-driven techniques which includes making predictions for individual process instances or overall process models. At the instance level, various novel techniques have been recently devised, tackling next activity, remaining time, and outcome prediction. At the model level, there is a notable void. It is the ambition of this paper to fill this gap. To this end, we develop a technique to forecast the entire process model from historical event data. A forecasted model is a will-be process model representing a probable future state of the overall process. Such a forecast helps to investigate the consequences of drift and emerging bottlenecks. Our technique builds on a representation of event data as multiple time series, each capturing the evolution of a behavioural aspect of the process model, such that corresponding forecasting techniques can be applied. Our implementation demonstrates the accuracy of our technique on real-world event log data.

==> 4b-result_table.tex <==
\begin{table}[htbp]
  \centering
  \resizebox{0.75\textwidth}{!}{
    \begin{tabular}{|c|l|ccc|ccc|ccc|}
\cmidrule{3-11}    \multicolumn{1}{r}{} &       & \multicolumn{3}{c|}{\textbf{BPI 12}} & \multicolumn{3}{c|}{\textbf{Sepsis}} & \multicolumn{3}{c|}{\textbf{RTFMP}} \\
    \multicolumn{1}{r}{} &       & \textbf{50} & \textbf{75} & \textbf{100} & \textbf{50} & \textbf{75} & \textbf{100} & \textbf{50} & \textbf{75} & \textbf{100} \\
    \midrule
    \multirow{5}[2]{*}{\begin{sideways}\textbf{equisize}\end{sideways}} & \textbf{nav} & 9.74  & 8.56  & 9.82  & 97.09 & 97.40 & 100.76 & 437.14 & \textbf{105.81} & 115.34 \\
          & \textbf{arima212} & 12.41 & 9.75  & 10.80 & NA    & \textbf{83.31} & \textbf{100.58} & \textbf{398.66} & NA    & NA \\
          & \textbf{ar2} & NA    & \textbf{8.45} & \textbf{9.62} & \textbf{97.04} & 97.40 & 100.76 & NA    & NA    & \textbf{110.14} \\
          & \textbf{hw} & \textbf{8.61} & 8.96  & 10.14 & 97.09 & 97.40 & 100.76 & 402.83 & 110.17 & 130.10 \\
          & \textbf{garch} & 11.47 & 8.60  & 10.17 & 97.09 & 97.40 & 100.76 & 426.71 & 109.79 & 117.15 \\
    \midrule
    \multicolumn{1}{|c|}{\multirow{5}[2]{*}{\begin{sideways}\textbf{equitemp}\end{sideways}}} & \textbf{nav} & 15.57 & 10.14 & 12.63 & 98.51 & 100.75 & NA    & 199.69 & 29.70 & 36.15 \\
          & \textbf{arima212} & NA    & 11.67 & \textbf{12.00} & \textbf{89.07} & \textbf{100.39} & NA    & \textbf{122.63} & \textbf{28.55} & \textbf{33.82} \\
          & \textbf{ar2} & NA    & \textbf{9.97} & 12.43 & 98.37 & 100.75 & NA    & NA    & 29.74 & NA \\
          & \textbf{hw} & \textbf{13.09} & 10.46 & 12.08 & 98.40 & 100.75 & NA    & 162.94 & 29.34 & 36.15 \\
          & \textbf{garch} & 17.80 & 10.29 & 12.71 & 95.75 & 100.75 & NA    & 199.13 & 30.44 & 36.00 \\
    \bottomrule
    \end{tabular}%
    }
    \caption{Overview of the mean percentage error in terms of entropic relevance.}
  \label{tab:result_table}%
\end{table}%


==> addon/macros.tex <==
%
% This one allows us to have a custom DESCRIPTION environment, in which numbers are preceded by a one-letter prefix.
% A short description can be added as an additional parameter to the begin-environment command.
% Successive references will have that very one-letter prefix + number with hyper-reference to it.
%
\RequirePackage{enumitem}
%
\def\requiprefix{T}
%
\newcounter{requicount}
\newlist{requidescr}{description}{1}
\setlist[requidescr,1]{%
	before={\setcounter{requicount}{0}%
		\renewcommand*\therequicount{\arabic{requicount}}},
	,font=\bfseries{\requiprefix}\stepcounter{requicount}\therequicount\normalfont.~\bfseries
}
%
% From https://tex.stackexchange.com/questions/1230/reference-name-of-description-list-item-in-latex
\makeatletter
\def\namedlabel#1{\begingroup
	\def\@currentlabel{\requiprefix\therequicount}%
	\phantomsection\label{#1}\endgroup
}
\makeatother
%
% Usage example:
% \begin{requidescr} % CUSTOM from CDC, with love
%   \item[\namedlabel{req:xaxis} Cluster on Y axis] Something more about that here.
% \end{requidescr}
% I especially like \ref{req:xaxis}.
